Tackling Heterogeneous Traffic in Multi-access Systems via Erasure Coded Servers

Most data generated by modern applications is stored in the cloud, and there is an exponential growth in the volume of jobs to access these data and perform computations using them. The volume of data access or computing jobs can be heterogeneous across different job types and can unpredictably change over time. Cloud service providers cope with this demand heterogeneity and unpredictability by over-provisioning the number of servers hosting each job type. In this paper, we propose the addition of erasure-coded servers that can flexibly serve multiple job types without additional storage cost. We analyze the service capacity region and the response time of such erasure-coded systems and compare them with standard uncoded replication-based systems currently used in the cloud. We show that coding expands the service capacity region, thus enabling the system to handle variability in demand for different data types. Moreover, we characterize the response time of the coded system in various arrival rate regimes. This analysis reveals that adding even a small number of coded servers can significantly reduce the mean response time, with a drastic reduction in regimes where the demand is skewed across different job types.

==> header.tex <==
\newif\ifmoment
%\momenttrue
\newif\iflong
\longtrue
\newif\ifNIPS
%\NIPStrue
\newif\ifShowDeprecated
%\ShowDeprecatedtrue
\newif\ifNotForSubmission
\NotForSubmissiontrue
%\documentclass[11pt]{article}


\ifNIPS

\PassOptionsToPackage{numbers,sort,compress}{natbib}
\usepackage{neurips_2019}

\usepackage[format=hang,font={footnotesize}]{caption}
\else
%\documentclass[11pt,letterpaper]{article}
\usepackage[papersize={8.5in,11in},margin=1in]{geometry}
\usepackage[numbers,sort,compress]{natbib} % flexible bibliography support
\usepackage[format=hang,font={footnotesize}]{caption}
\fi
\usepackage[title]{appendix}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
% \usepackage{algorithmic}
% \usepackage{subfigure}
\usepackage{wrapfig}
\usepackage{color}
\usepackage{enumitem}
\usepackage{parskip}

\usepackage{graphicx}
\usepackage{dirtytalk}
\usepackage{complexity}
\usepackage{algorithm}
%\usepackage{algorithmic}
\usepackage{setspace}
\usepackage{subcaption}

\usepackage{tcolorbox}

\usepackage{url}
\usepackage{graphicx}
\usepackage{color}
\usepackage{algorithm} % pseudocode support
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}
%\renewcommand\algorithmiccomment[1]{ \hfill $\diamond$ \ {\footnotesize \em #1} }

\usepackage{xspace}
\usepackage{dsfont} % to allow mathds (mathbb)
\usepackage{pifont} % to allow circled numbers
\usepackage{bbm}
\usepackage{comment}
\usepackage{float}
\usepackage{listings}
\usepackage{xcolor}
% \usepackage[colorinlistoftodos]{todonotes}

\newtheorem{innercustomthm}{Theorem}
\newenvironment{stheorem}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
\newtheorem{innercustomlemma}{Lemma}
\newenvironment{slemma}[1]
  {\renewcommand\theinnercustomlemma{#1}\innercustomlemma}
  {\endinnercustomlemma}
\newtheorem{innercustomclaim}{Claim}
\newenvironment{sclaim}[1]
  {\renewcommand\theinnercustomclaim{#1}\innercustomclaim}
  {\endinnercustomclaim}
\newtheorem{ctheorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Theorem}[section]
\newtheorem{claim}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{ccorollary}[ctheorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{cconcept}{Concept}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{thm}[theorem]{Theorem}
\newtheorem{lem}[lemma]{Lemma}
\newtheorem{clm}[claim]{Claim}
\newtheorem{property}[theorem]{Property}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{conj}[theorem]{Conjecture}
\newtheorem*{assumption*}{Assumption}
\newtheorem*{question*}{Question}


\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}


\newreptheorem{theorem}{Theorem}
\newreptheorem{lemma}{Lemma}
\newreptheorem{proposition}{Proposition}
\newreptheorem{claim}{Claim}
\newreptheorem{definition}{Definition}
%\newreptheorem{problem}{Problem}


%\ifCOLT\else
\theoremstyle{definition}
%\fi
\newtheorem{construction}[theorem]{Construction}
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{problem}[theorem]{Problem} %%% added by Zhao
\newtheorem{param}[theorem]{Parameter}
\newtheorem*{defn}{Definition}
\newtheorem*{exmp}{Example}

\captionsetup[subfigure]{subrefformat=simple,labelformat=simple}
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
 
\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=none,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}
\lstset{style=mystyle}
%\ifCOLT\else
\theoremstyle{remark}
%\fi
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem*{note}{Notation}
\newtheorem{case}{Case}
\newtheorem*{rem}{Remark}
\newtheorem*{hnote}{Historical Note}
\newtheorem*{ack}{Acknowledgments}
\newtheorem{example}[theorem]{Example}

\numberwithin{equation}{section}

\newenvironment{proofsketch}{\noindent{\it Proof sketch.}\hspace*{1em}}{\qed\bigskip}

%\ifCOLT\else
\renewcommand{\qedsymbol}{\hfill{\Large $\square$}}
%\fi
\newcommand{\bqed}{\hfill{\Large $\blacksquare$}}



\newcommand{\namedref}[2]{\mbox{\hyperref[#2]{#1~\ref*{#2}}}}

\newcommand{\chapterref}[1]{\namedref{Chapter}{#1}}
\newcommand{\sectionref}[1]{\namedref{Section}{#1}}
\newcommand{\appendixref}[1]{\namedref{Appendix}{#1}}
\newcommand{\theoremref}[1]{\namedref{Theorem}{#1}}
\newcommand{\factref}[1]{\namedref{Fact}{#1}}
\newcommand{\remarkref}[1]{\namedref{Remark}{#1}}
\newcommand{\definitionref}[1]{\namedref{Definition}{#1}}
\newcommand{\figureref}[1]{\namedref{Figure}{#1}}
\newcommand{\figurerefb}[2]{\mbox{\hyperref[#1]{Figure~\ref*{#1}#2}}}
\newcommand{\tableref}[1]{\namedref{Table}{#1}}
\newcommand{\lemmaref}[1]{\namedref{Lemma}{#1}}
\newcommand{\claimref}[1]{\namedref{Claim}{#1}}
\newcommand{\propositionref}[1]{\namedref{Proposition}{#1}}
\newcommand{\corollaryref}[1]{\namedref{Corollary}{#1}}
\newcommand{\constructionref}[1]{\namedref{Construction}{#1}}
\newcommand{\itemref}[1]{\namedref{Item}{#1}}
\newcommand{\propertyref}[1]{\namedref{Property}{#1}}
\newcommand{\protocolref}[1]{\namedref{Protocol}{#1}}
\newcommand{\algorithmref}[1]{\namedref{Algorithm}{#1}}
\newcommand{\assumptionref}[1]{\namedref{Assumption}{#1}}
\newcommand{\conceptref}[1]{\namedref{Concept}{#1}}
\newcommand{\stepref}[1]{\namedref{Step}{#1}}
\newcommand{\paramref}[1]{\namedref{Parameter}{#1}}
\newcommand{\footnoteref}[1]{\namedref{Footnote}{#1}}
\newcommand{\equationref}[1]{\mbox{\hyperref[#1]{(\ref*{#1})}}}
\renewcommand{\eqref}{\equationref}
%\newcommand{\equationref}[1]{\namedref{Equation}{#1}}
\newcommand{\exampleref}[1]{\namedref{Example}{#1}}
\newcommand{\plineref}[1]{\namedref{Line}{#1}}


\newcommand{\var}{\mathbf{Var}}
\newcommand{\new}{{(\mathsf{new})}}

\newcommand{\argmax}{\operatornamewithlimits{arg\,max}}
\newcommand{\argmin}{\operatornamewithlimits{arg\,min}}
\DeclareMathOperator*{\sign}{sign}

\makeatletter
% LeftRightArrow
\newcommand\xLongLeftRightArrow[2][]%
  {\ext@arrow 0099{\LongLeftRightArrowfill@}{#1}{#2}}
\def\LongLeftRightArrowfill@
  {\arrowfill@\Leftarrow\Relbar\Rightarrow}
% Rightarrow
\newcommand\xLongRightArrow[2][]%
  {\ext@arrow 0099{\LongRightArrowfill@}{#1}{#2}}
\def\LongRightArrowfill@
  {\arrowfill@\Relbar\Relbar\Rightarrow}
\makeatother


% defeq
\iflong
\newcommand{\defeq}{\stackrel{\mathrm{\scriptscriptstyle def}}{=}}
\newcommand{\defem}[1]{\textsf{#1}}
\else
\newcommand{\defeq}{:=}
\newcommand{\defem}[1]{\emph{\textsf{\small #1}}}
\fi

% paragraph headings
\newcommand{\loss}{\mathbf{Obj}}
\newcommand{\lossh}{\tilde{\mathbf{Obj}}}
\newcommand{\lloss}{\mathbf{Loss}}
\newcommand{\llossh}{\tilde{\mathbf{Loss}}}
\newcommand{\xE}{{\mathsf{xE}}}
\newcommand{\CE}{{\mathsf{CE}}}
\newcommand{\reg}{\mathbf{Reg}}
\renewcommand{\bar}{\overline}
\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\emptyset}{\varnothing}

\newcommand{\da}{\text{\ding{172}}\xspace}
\newcommand{\db}{\text{\ding{173}}\xspace}
\newcommand{\dc}{\text{\ding{174}}\xspace}
\newcommand{\dd}{\text{\ding{175}}\xspace}
\newcommand{\de}{\text{\ding{176}}\xspace}
\newcommand{\df}{\text{\ding{177}}\xspace}
\newcommand{\dg}{\text{\ding{178}}\xspace}

\newcommand{\tW}{\tilde{W}}
\newcommand{\SUM}{\mathbf{Sum}}
\newcommand{\SYM}{\mathbf{Sym}}
\newcommand{\Fstar}{G^\star}
\newcommand{\tA}{\tilde{A}}
\newcommand{\tw}{\tilde{w}}
\newcommand{\ta}{\tilde{a}}
\newcommand{\tg}{\tilde{g}}
\newcommand{\tD}{\tilde{D}}

\newcommand{\Ws}{W^\divideontimes}
\newcommand{\ws}{w^\divideontimes}

%\newcommand{\bWz}{{\bW^{(0)}}}
%\newcommand{\bVz}{{\bV^{(0)}}}
%\renewcommand{\star}{\divideontimes}
\newcommand{\bWbar}{\breve{\bW}}
\newcommand{\bWhat}{\bar{\bar{\bW}}}
\newcommand{\bWp}{\bW'}
\newcommand{\bWg}{\bW^\star}
\newcommand{\kappap}{\tilde{\kappa}}
\newcommand{\kb}{\bar{k}}
\newcommand{\Bb}{\bar{B}}
\newcommand{\bVg}{\bV^\star}
\newcommand{\bVgg}{\bV^{\star,w}}
\newcommand{\bDp}{\bD'}
\newcommand{\bDpp}{\bD''}
\newcommand{\bDz}{\tilde{\bD}}
\newcommand{\bDbar}{\breve{\bD}}
\newcommand{\bDs}{\bD^{\mathsf{0/1}}}
\newcommand{\hp}{h'}
\newcommand{\hz}{\tilde{h}}
\renewcommand{\hbar}{\breve{h}}
\newcommand{\gp}{g'}
\newcommand{\gz}{g^{(0)}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\gbar}{\breve{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\lhat}{\hat{\loss}}
\newcommand{\lbar}{\breve{\loss}}
\newcommand{\done}{\mathds{1}}
\newcommand{\II}{\mathds{1}}
\newcommand{\tauS}{\tau_\triangledown}
\newcommand{\xs}{x^\star}
\newcommand{\ys}{y^\star}
\newcommand{\dx}{{d_x}}
\newcommand{\vepss}{\veps_{\mathsf{s}}}
\newcommand{\vepsx}{\veps_x}
\newcommand{\vepsc}{\veps_c}
\newcommand{\vepse}{\veps_e}
\newcommand{\complexity}{\mathfrak{C}}
\newcommand{\complexitys}{\mathfrak{C}_\mathfrak{s}}
\newcommand{\complexityE}{\mathfrak{C}_\veps}
\newcommand{\complexityalpha}{\mathfrak{C}_\alpha}
\newcommand{\complexitytalpha}{\mathfrak{C}_{\tilde{\alpha}}}
\newcommand{\obj}{\mathsf{Obj}}

\newcommand{\TauZeroBound}{\rhob^{100}}
\newcommand{\rhob}{\varrho}
\newcommand{\rhobVal}{n L d \delta^{-1} \log (m/\veps)}

\newcommand{\veps}{\varepsilon}
\newcommand{\GS}{\mathsf{GS}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\sgn}{\mathsf{sgn}}
\newcommand{\lmax}{\lambda_{\max}}
\newcommand{\lmin}{\lambda_{\min}}
\newcommand{\Va}{\mathcal{V}}

\newcommand{\out}{\mathsf{out}}
\newcommand{\outK}{\mathfrak{K}}
\newcommand{\outF}{\mathfrak{F}}
\newcommand{\outa}{\mathsf{out}_1}
\newcommand{\Lg}{\mathfrak{L}_\cG}
\newcommand{\Bf}{\mathfrak{B}_\cF}
\newcommand{\Bg}{\mathfrak{B}_\cG}
\newcommand{\Bfg}{\mathfrak{B}_{\cF\circ \cG}}
\newcommand{\az}{a}
\newcommand{\bz}{b}
\newcommand{\ReLU}{\sigma}



\newcommand{\nbr}[1]{{\left\| {#1} \right\|}}

\renewcommand{\E}{\operatornamewithlimits{\mathbb{E}}}
\renewcommand{\Pr}{\operatornamewithlimits{\mathbf{Pr}}}
\newcommand{\Lap}{\mathcal{L}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Real}{\mathbb{R}}
%\newcommand{\dd}{\rm{d}}
%\newcommand{\PP}{\rm{P}}
\newcommand{\set}[1]{\mathcal{#1}}
\newcommand{\NumContext}{N}
%\newcommand{\diag}{\textsf{diag}}

\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cF}{\mathcal{F}}
%\newcommand{\cS}{\mathcal{S}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cI}{\mathcal{I}}

\newcommand{\N}{\mathcal{N}}

\newcommand{\matrixstyle}{\mathbf}
\newcommand{\bF}{\matrixstyle{F}}
\newcommand{\bE}{\matrixstyle{E}}
\newcommand{\bC}{\matrixstyle{C}}
\newcommand{\bN}{\matrixstyle{N}}
\newcommand{\bM}{\matrixstyle{M}}
\newcommand{\bA}{\matrixstyle{A}}
\newcommand{\bAg}{\matrixstyle{A}^\star}
\newcommand{\bB}{\matrixstyle{B}}
\newcommand{\bX}{\matrixstyle{X}}
\newcommand{\bY}{\matrixstyle{Y}}
\newcommand{\bU}{\matrixstyle{U}}
\newcommand{\bu}{\matrixstyle{u}}
\newcommand{\bV}{\matrixstyle{V}}
\newcommand{\bL}{\matrixstyle{L}}
\newcommand{\btV}{\widetilde{\matrixstyle{V}}}
\newcommand{\bG}{\matrixstyle{G}}
\newcommand{\bH}{\matrixstyle{H}}
\newcommand{\bO}{\matrixstyle{O}}
\newcommand{\bP}{\matrixstyle{P}}
\newcommand{\bQ}{\matrixstyle{Q}}
\newcommand{\btE}{\widetilde{\matrixstyle{E}}}
\newcommand{\bD}{\matrixstyle{D}}
\newcommand{\bJ}{\matrixstyle{J}}
\newcommand{\bK}{\matrixstyle{K}}
\newcommand{\bR}{\matrixstyle{R}}
\newcommand{\btR}{\matrixstyle{\widetilde{R}}}
\newcommand{\btQ}{\matrixstyle{\widetilde{Q}}}
\newcommand{\bS}{\matrixstyle{S}}
\newcommand{\bI}{\matrixstyle{I}}
\newcommand{\btM}{\widetilde{\matrixstyle{M}}}
\newcommand{\bT}{\matrixstyle{T}}
\newcommand{\bTb}{\matrixstyle{T}_{\bot}}
\newcommand{\btXb}{\widetilde{\matrixstyle{X}}_{\bot}}
\newcommand{\btX}{\widetilde{\matrixstyle{X}}}
\newcommand{\bbX}{\overline{\matrixstyle{X}}}
\newcommand{\btY}{\widetilde{\matrixstyle{Y}}}
\newcommand{\btYb}{\widetilde{\matrixstyle{Y}}_{\bot}}
\newcommand{\bbY}{\overline{\matrixstyle{Y}}}
\newcommand{\btSigma}{\widetilde{\matrixstyle{\Sigma}}}
\newcommand{\bZ}{\matrixstyle{Z}}
\newcommand{\bW}{\matrixstyle{W}}
\newcommand{\bOne}{\matrixstyle{1}}

\newcommand{\ckappa}{\tau}
\newcommand{\bSigma}{\matrixstyle{\Sigma}}
\newcommand{\bDelta}{\matrixstyle{\Delta}}
%\newcommand{\bMg}{\matrixstyle{M}^*}
\newcommand{\bNoise}{\matrixstyle{N}}
\newcommand{\bGamma}{\matrixstyle{\Gamma}}
\newcommand{\bLambda}{\matrixstyle{\Lambda}}

\newcommand{\tY}{\widetilde{\matrixstyle{Y}}}

\newcommand{\bbSigma}{\overline{\matrixstyle{\Sigma}}}

\newcommand{\dmaxp}{D_2}
\newcommand{\dmax}{D_1}
\newcommand{\sP}{\set{P}}

%\newcommand{\Us}{(\bU^*)}
%\newcommand{\Vs}{(\bV^*)}

\newcommand{\bUb}{\matrixstyle{U}_{\bot}}
\newcommand{\bVb}{\matrixstyle{V}_{\bot}}
\newcommand{\bXb}{\matrixstyle{X}_{\bot}}
\newcommand{\bYb}{\matrixstyle{Y}_{\bot}}
\newcommand{\bOneb}{\matrixstyle{1}_{\bot}}


\newcommand{\lambdal}{\underline{\lambda}}
\newcommand{\lambdau}{\overline{\lambda}}
\newcommand{\sigmas}{{\sigma}_s}
\newcommand{\sigmal}{{\sigma}_l}
\newcommand{\sigmat}{\tilde{\sigma}}


\newcommand{\cds}{\textsf{dist}_c}

\newcommand{\leftll}{\left\|}
\newcommand{\rightll}{\right\|}
%\newcommand{\hp}{\odot}
%\newcommand{\ortho}{\textsf{O}}
\newcommand{\QR}{\textsf{QR}}
\newcommand{\SVD}{\textsf{SVD}}
%\newcommand{\rank}{k}
\newcommand{\trace}{\bold{Tr}}
\newcommand{\tr}{\trace}
\newcommand{\diag}{\bold{diag}}
\newcommand{\Tr}{\trace}
\newcommand{\Rad}{\mathfrak{R}}
\newcommand{\OPT}{\mathsf{OPT}}

\newcommand{\AlgRInitial}{\textsf{RandInitial}}
\newcommand{\AlgInitial}{\textsf{SVDInitial}}
\newcommand{\AlgWhitening}{\textsf{Whitening}}
\newcommand{\AlgMain}{\textsf{Alt}}
\newcommand{\AlgClip}{\textsf{Clip}}

\newcommand{\incoherentpartial}{\rho}
\newcommand{\incoherentfull}{\mu}
\newcommand{\valupdate}{\textsf{val}}
\newcommand{\valdelta}{\textsf{c}}

\newcommand{\subs}{\text{SS}}
\newcommand{\subsr}{\text{RSS}}
\newcommand{\subsc}{\text{CSS}}

\newcommand{\tx}{\tilde{x}} % the decoding before threshold
\newcommand{\xp}{{x'}} % the decoding for the shadow sample
\newcommand{\yp}{{y'}} % the shadow sample
\newcommand{\thres}[2]{\phi_{#1}\rbr{#2}} % the threshold
\newcommand{\ntopic}{K}
\newcommand{\nword}{n}
\newcommand{\damp}{R}
\newcommand{\ntdoc}{s} % number of topics in each document
\newcommand{\rbr}[1]{\left(#1\right)} % brackets
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\replace}{\text{Rep}}
\newcommand{\postime}[2]{{#1}^{(#2)}_{+}}
\newcommand{\negtime}[2]{{#1}^{(#2)}_{-}}
\newcommand{\titime}[2]{{#1}^{(#2)}}

\newcommand{\pt}[1]{\postime{#1}{t}}
\newcommand{\nt}[1]{\negtime{#1}{t}}
\newcommand{\ti}[1]{\titime{#1}{t}}

\newcommand{\pto}[1]{\postime{#1}{t+1}}
\newcommand{\nto}[1]{\negtime{#1}{t+1}}
\newcommand{\tio}[1]{\titime{#1}{t+1}}
\newcommand{\sym}[1]{\left\|{#1}\right\|_{\mbox{sym}}}

\newcommand{\xmin}{x_{\textrm{min}}} 
\newcommand{\xexpc}{c_0} 
\newcommand{\corr}{c_1}
\newcommand{\minprob}{c_3}
\newcommand{\eqnref}[1]{(\ref{#1})} 
\newcommand{\sigmac}{C}
\newcommand{\sigmamax}{\Sigma_{\max}}

\newcommand{\AlgDecode}{\textsf{Decode}}

\newcommand{\AlgRen}{\textsf{Renormalization}}
\newcommand{\valupE}{c}
\newcommand{\correlation}{\mathcal{C}}
\newcommand{\corre}{\mathcal{C}}



\DeclareMathOperator*{\prox}{prox}


\usepackage{lineno}
\def\linenumberfont{\normalfont\small}

\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}
